Uniform Inference for Kernel Density Estimators with Dyadic Data

Dyadic data is often encountered when quantities of interest are associated with the edges of a network. As such it plays an important role in statistics, econometrics and many other data science disciplines. We consider the problem of uniformly estimating a dyadic Lebesgue density function, focusing on nonparametric kernel-based estimators taking the form of dyadic empirical processes. Our main contributions include the minimax-optimal uniform convergence rate of the dyadic kernel density estimator, along with strong approximation results for the associated standardized and Studentized $t$-processes. A consistent variance estimator enables the construction of valid and feasible uniform confidence bands for the unknown density function. We showcase the broad applicability of our results by developing novel counterfactual density estimation and inference methodology for dyadic data, which can be used for causal inference and program evaluation. A crucial feature of dyadic distributions is that they may be "degenerate" at certain points in the support of the data, a property making our analysis somewhat delicate. Nonetheless our methods for uniform inference remain robust to the potential presence of such points. For implementation purposes, we discuss inference procedures based on positive semi-definite covariance estimators, mean squared error optimal bandwidth selectors and robust bias correction techniques. We illustrate the empirical finite-sample performance of our methods both in simulations and with real-world trade data, for which we make comparisons between observed and counterfactual trade distributions in different years. Our technical results concerning strong approximations and maximal inequalities are of potential independent interest.

==> preamble.tex <==
% Packages
% -------------------------------

\usepackage{float}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage[hypertexnames=false]{hyperref}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathrsfs}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage[margin=1in]{geometry}
\usepackage{multirow}
\usepackage{microtype}
\usepackage{titlesec}
\usepackage[longnamesfirst]{natbib}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{stackengine,scalerel}
\usepackage{tocloft}
\usepackage[boxruled,
  linesnumbered,
  commentsnumbered,
  procnumbered,
]{algorithm2e}

% Document settings
% -------------------------------

%\setlength{\bibsep}{8pt}
\hypersetup{pdfborder = {0 0 0},colorlinks=true,linkcolor=blue,urlcolor=blue,citecolor=blue}
\setcounter{tocdepth}{2}
\cftsetindents{section}{0em}{3em}
\cftsetindents{subsection}{2em}{4em}

% Macros
% -------------------------------

% Math operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\ABias}{ABias}
\DeclareMathOperator{\AIMSE}{AIMSE}
\DeclareMathOperator{\AMSE}{AMSE}
\DeclareMathOperator{\AVar}{AVar}
\DeclareMathOperator{\Ber}{Ber}
\DeclareMathOperator{\Bias}{Bias}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\diverge}{div}
\DeclareMathOperator{\Env}{Env}
\DeclareMathOperator{\IQR}{IQR}
\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\Leb}{Leb}
\DeclareMathOperator*{\logistic}{logistic}
\DeclareMathOperator{\ME}{ME}
\DeclareMathOperator{\MSE}{MSE}
\DeclareMathOperator{\IMSE}{IMSE}
\DeclareMathOperator{\ROT}{ROT}
\DeclareMathOperator{\symconv}{symconv}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator*{\esssup}{ess\,sup}

% Single characters
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bV}{\ensuremath{\mathbf{V}}}
\newcommand{\bW}{\ensuremath{\mathbf{W}}}
\newcommand{\bX}{\ensuremath{\mathbf{X}}}
\newcommand{\bY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bZ}{\ensuremath{\mathbf{Z}}}
\renewcommand{\P}{\ensuremath{\mathbb{P}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cPd}{\ensuremath{\mathcal{P}_{\mathrm{d}}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\bbN}{\ensuremath{\mathbb{N}}}
\newcommand{\CH}{\ensuremath{C_\mathrm{H}}}
\newcommand{\Cd}{\ensuremath{C_\mathrm{d}}}
\newcommand{\CL}{\ensuremath{C_\mathrm{L}}}
\newcommand{\Ck}{\ensuremath{C_\mathrm{k}}}
\newcommand{\objective}{\ensuremath{\mathrm{obj}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\I}{\ensuremath{\mathbb{I}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\T}{\ensuremath{\mathsf{T}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}

\newcommand{\flbeta}{\ThisStyle{%
    \ensurestackMath{\stackengine{-0.5\LMpt}{\SavedStyle \beta}{\SavedStyle {\rule{3.7\LMpt}{0.3\LMpt}}}
      {U}{c}{F}{F}{S}}\vphantom{\beta}}}

\newcommand{\fln}{\ThisStyle{%
    \ensurestackMath{\stackengine{0.8\LMpt}{\SavedStyle n}{\SavedStyle {\rule{4.2\LMpt}{0.3\LMpt}}}
      {U}{c}{F}{F}{S}}\vphantom{n}}}

% Other macros
\newcommand{\maxi}{\ensuremath{\mathrm{max}}}
\newcommand{\mini}{\ensuremath{\mathrm{min}}}
\DeclareMathOperator*{\minimize}{minimize:}
\DeclareMathOperator*{\subjectto}{subject\ to:}
\newcommand{\dprime}{\ensuremath{\prime\prime}}
\newcommand{\tprime}{\ensuremath{\prime\prime\prime}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\Lip}{\mathrm{Lip}}
\newcommand{\Data}{\textup{Data}}
\newcommand{\diff}[1]{\,\mathrm{d}#1}
\newcommand{\TODO}[1]{\textcolor{red}{\textsc{TODO}: #1}}
\newcommand{\Dl}{\ensuremath{D_{\textup{lo}}}}
\newcommand{\Du}{\ensuremath{D_{\textup{up}}}}

% Paragraph formatting
% -------------------------------
\titleformat
{\paragraph}
[hang]
{\bfseries\upshape}
{}
{0pt}
{}
[] % command% shape% format% label% sep% before-code% after-code

\titlespacing*{\paragraph}{0pt}{6pt}{0pt}

\newcounter{proofparagraphcounter}

\newcommand{\proofparagraph}[1]{
  \refstepcounter{proofparagraphcounter}%
  \paragraph{Part \theproofparagraphcounter : #1}}%

% Environments
% -------------------------------

\newtheoremstyle{break}%
{\topsep}{\topsep}%
{\itshape}{}%
{\bfseries}{}%
{\newline}%
%
% For theorems not in TOC
{}%
%
% For theorems in TOC
%{\thmname{#1}\thmnumber{ #2}%
%\thmnote{ \rm(#3)\addcontentsline{toc}{subsubsection}{{\it#1 #2}: #3}}}

\newtheoremstyle{breakplainproof}
{\topsep}{\topsep}%
{}{}%
{\bfseries}{}%
{\newline}%
%
% For proofs not in TOC
{}%
%
% For proofs in TOC
%{\thmname{#1}\thmnumber{ #2}%
%\thmnote{ \rm(#3)\addcontentsline{toc}{subsubsection}{{\it#1}: #3}}}

\theoremstyle{break}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{definition}{Definition}

\theoremstyle{breakplainproof}
\let\proof\relax
\newtheorem*{proof}{Proof}
\AtBeginEnvironment{proof}{\setcounter{proofparagraphcounter}{0}}%
\AtEndEnvironment{proof}{\null\hfill\qedsymbol}%

\theoremstyle{remark}
\newtheorem*{remark}{Remark}

% include "SA"
\renewcommand{\thelemma}{SA\arabic{lemma}}
\renewcommand{\thetheorem}{SA\arabic{theorem}}
\renewcommand{\theassumption}{SA\arabic{assumption}}
\renewcommand{\thedefinition}{SA\arabic{definition}}
\renewcommand{\thesection}{SA\arabic{section}}

% Algorithms
% -------------------------------

\DontPrintSemicolon
\makeatletter
\renewcommand{\SetKwInOut}[2]{\sbox\algocf@inoutbox{\KwSty{#2}\algocf@typo:}\expandafter\ifx\csname InOutSizeDefined\endcsname\relax \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}\sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}\else
    \ifdim\wd\algocf@inoutbox>\inoutsize
      \setlength{\inoutsize}{\wd\algocf@inoutbox}\sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}\fi
  \fi
  \algocf@newcommand{#1}[1]{\ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\everypar={\relax}}{\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo:\hfill}~##1\par}\algocf@linesnumbered }}\makeatother
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\setlength{\algomargin}{2em}

